Being-H0.7: A Latent World-Action Model from Egocentric Videos

Visual-Language-Action models (VLAs) have advanced generalist robot control by mapping multimodal observations and language instructions directly to actions, but sparse action supervision often encourages shortcut mappings rather than representations of dynamics, contact, and task progress. Recent world-action models introduce future prediction through video rollouts, yet pixel-space prediction is a costly and indirect substrate for control, as it may model visual details irrelevant to action generation and introduces substantial training or inference overhead. We present Being-H0.7, a latent world-action model that brings future-aware reasoning into VLA-style policies without generating future frames. Being-H0.7 inserts learnable latent queries between perception and action as a compact reasoning interface, and trains them with a future-informed dual-branch design: a deployable prior branch infers latent states from the current context, while a training-only posterior branch replaces the queries with embeddings from future observations. Jointly aligning the two branches at the latent reasoning space leads the prior branch to reason future-aware, action-useful structure from current observations alone. At inference, Being-H0.7 discards the posterior branch and performs no visual rollout. Experiments across six simulation benchmarks and diverse real-world tasks show that Being-H0.7 achieves state-of-the-art or comparable performance, combining the predictive benefits of world models with the efficiency and deployability of direct VLA policies.

==> table/abl_pretrain_multi_task.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Impact ablation of human-centric learning in multi-task 5-shot adaptation.} 
In contrast to the single-task setup, the model is jointly trained on data from all four task suites and subsequently evaluated on each individually. 
\textbf{Native VLM}: Initialized from the original large multimodal model. 
\textbf{Human-Centric}: Initialized with our human-centric pretrained weights.
This multi-task protocol serves to rigorously assess the generalization capabilities and robustness of VLAs under diverse cross-task scenarios.}
\label{tab:abl_pretrain_multi}
\small
\setlength{\tabcolsep}{9pt} 
\begin{tabular}{ll ccccc}
\toprule
\multicolumn{2}{c}{\textbf{Model Configuration}} & \multicolumn{5}{c}{\textbf{Multi-task-suite LIBERO 5-Shot Success Rate (\%)}} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-7}
\textbf{Frozen Components} & \textbf{Initialization} & \textbf{L-Spatial} & \textbf{L-Object} & \textbf{L-Goal} & \textbf{L-Long} & \textbf{Avg.} \\
\midrule

% Group 1: All Frozen
\multirow{3}{*}{\textbf{Und + Proj + ViT}} 
    & Native VLM & 61.6 & 77.0 & 68.0 & 36.0 & 60.7 \\
    & Human-Centric & 80.8 & 81.8 & 74.4 & 52.4 & 72.4 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+19.2} & \textbf{+4.8} & \textbf{+6.4} & \textbf{+16.4} & \textbf{+11.7} \\
\addlinespace[0.6em]

% Group 2: Und + ViT
\multirow{3}{*}{\textbf{Und + ViT}}       
    & Native VLM & 78.4 & 84.8 & 71.4 & 38.6 & 68.3 \\
    & Human-Centric & 83.6 & 82.6 & 80.8 & 59.2 & 76.6 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+5.2} & \textcolor{red}{-2.2} & \textbf{+9.4} & \textbf{+20.6} & \textbf{+8.3} \\
\addlinespace[0.6em]
\midrule

% Group 3: Und Only
\multirow{3}{*}{\textbf{Und Only}}             
    & Native VLM & 75.8 & 84.2 & 71.2 & 59.8 & 72.8 \\
    & Human-Centric & 85.2 & 90.6 & 84.2 & 68.4 & 82.1 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+9.4} & \textbf{+6.4} & \textbf{+13.0} & \textbf{+8.6} & \textbf{+9.3} \\
\addlinespace[0.6em]

% Group 4: Proj + ViT
\multirow{3}{*}{\textbf{Proj + ViT}}      
    & Native VLM & 87.6 & 91.0 & 82.2 & 62.6 & 80.9 \\
    & Human-Centric & 89.6 & 88.8 & 89.6 & 65.8 & 83.5 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+2.0} & \textcolor{red}{-2.2} & \textbf{+7.4} & \textbf{+3.2} & \textbf{+2.6} \\
\addlinespace[0.6em]

% Group 5: Full Fine-tuning
\multirow{3}{*}{\textbf{None (Full FT)}}  
    & Native VLM & 87.8 & 94.6 & 82.6 & 71.4 & 84.1 \\
    & Human-Centric & 88.8 & 90.2 & 85.4 & 76.0 & 85.1 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+1.0} & \textcolor{red}{-4.4} & \textbf{+2.8} & \textbf{+4.6} & \textbf{+1.0} \\
\bottomrule
\end{tabular}
\end{table*}



==> table/abl_pretrain_single_task.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Impact of human-centric learning in single-task 5-shot adaptation.} 
We investigate this by selectively freezing key architectural components.
\textbf{Native VLM}: Initialized from the original large multimodal model. 
\textbf{Human-Centric}: Initialized with our human-centric pretrained weights.
The action expert remains trainable in all settings.
$\Delta$ denotes the absolute performance gain.
}
\label{tab:abl_pretrain_single}
\small
\setlength{\tabcolsep}{9pt}
\begin{tabular}{ll ccccc}
\toprule
\multicolumn{2}{c}{\textbf{Model Configuration}} & \multicolumn{5}{c}{\textbf{Single-Task LIBERO 5-Shot Success Rate (\%)}} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-7}
\textbf{Frozen Components} & \textbf{Initialization} & \textbf{L-Spatial} & \textbf{L-Object} & \textbf{L-Goal} & \textbf{L-Long} & \textbf{Avg.} \\
\midrule

% Group 1: Full Freeze
\multirow{3}{*}{\textbf{Und + Proj + ViT}} 
    & Native VLM & 67.8 & 76.8 & 57.2 & 29.8 & 57.9 \\
    & Human-Centric & 78.6 & 78.9 & 72.6 & 46.2 & 69.0 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+10.8} & \textbf{+2.1} & \textbf{+15.4} & \textbf{+16.4} & \textbf{+11.1} \\
\addlinespace[0.6em]

% Group 2: Und + ViT (Highlight)
\multirow{3}{*}{\textbf{Und + ViT}}       
    & Native VLM & 70.6 & 50.0 & 67.0 & 17.4 & 51.3 \\
    & Human-Centric & 85.0 & 84.2 & 80.0 & 59.0 & 77.1 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+14.4} & \textbf{+34.4} & \textbf{+13.0} & \textbf{+41.6} & \textbf{+25.8} \\
\addlinespace[0.6em]
\midrule 

% Group 3: Und Only
\multirow{3}{*}{\textbf{Und Only}}             
    & Native VLM & 78.4 & 84.8 & 62.0 & 49.2 & 68.6 \\
    & Human-Centric & 83.2 & 79.6 & 74.0 & 63.6 & 75.1 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+4.8} & \textcolor{red}{-5.2} & \textbf{+12.0} & \textbf{+14.4} & \textbf{+6.5} \\
\addlinespace[0.6em]

% Group 4: Proj + ViT
\multirow{3}{*}{\textbf{Proj + ViT}}      
    & Native VLM & 87.2 & 86.6 & 80.8 & 58.0 & 78.2 \\
    & Human-Centric & 86.2 & 86.2 & 84.6 & 66.8 & 81.0 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textcolor{red}{-1.0} & \textcolor{red}{-0.4} & \textbf{+3.8} & \textbf{+8.8} & \textbf{+2.8} \\
\addlinespace[0.6em]

% Group 5: Fully Trainable
\multirow{3}{*}{\textbf{None (Full FT)}}  
    & Native VLM & 84.2 & 83.6 & 75.0 & 65.8 & 77.2 \\
    & Human-Centric & 87.2 & 91.4 & 81.6 & 66.8 & 81.8 \\
    \rowcolor{BlockA!30}
    & \textbf{Gain ($\Delta$)} & \textbf{+3.0} & \textbf{+7.8} & \textbf{+6.6} & \textbf{+1.0} & \textbf{+4.6} \\
\bottomrule
\end{tabular}
\end{table*}


==> table/embodiment_list.tex <==
\begin{table*}[h!]
\centering
\small 
\setlength{\tabcolsep}{6pt} 
\renewcommand{\arraystretch}{1.05} 
 
\caption{\textbf{Statistical overview of robot manipulation data in UniHand-2.0}. 
The corpus aggregates demonstrations across \textbf{30 distinct embodiments}, totaling \textbf{14,000 hours} of interaction.
The dataset is characterized by high diversity in camera views, kinematic structures, and operational environments, categorized by end-effector type---``Grp'' (parallel gripper) vs. ``Dex'' (dexterous hand), and data source---``Real'' (physical world) vs. ``Sim'' (simulation).}
\label{tab:robot_data}
 
\begin{tabular}{@{}l l c c r@{}}
\toprule
\textbf{Robot Type} & \textbf{Camera Views} & \textbf{EEF Type} & \textbf{Source} & \textbf{Hours} \\ 
\midrule
 
% --- Group 1 ---
\multicolumn{5}{l}{\textit{\textbf{Single-Arm Robots}}} \\ 
\addlinespace[0.2em] 
Franka        & ego, 3rd$\times$2, wrist & Grp/Dex & Real/Sim & 2196.4 \\ 
Google Robot  & ego, 3rd                 & Grp     & Real/Sim & 1195.2 \\ 
Kuka-iiwa     & ego, 3rd                 & Grp     & Real/Sim & 338.2 \\ 
WidowX        & 3rd$\times$2, wrist      & Grp     & Real/Sim & 305.2 \\ 
Xarm7 Robot   & top, 3rd                 & Grp     & Real/Sim & 594.4 \\ 
UR5E           & 3rd, wrist               & Grp     & Real/Sim & 208.3 \\ 
Hello Stretch & ego, 3rd                 & Grp     & Real     & 270.3 \\ 
Kinova Jaco          & 3rd$\times$3             & Grp     & Real/Sim & 194.6 \\ 
Kinova Gen3       & 3rd$\times$3             & Grp     & Sim      & 197.4 \\ 
Sawyer        & 3rd                      & Grp     & Sim      & 196.1 \\ 
Cobotta       & 3rd                      & Grp     & Real     & 10.6 \\ 
DLR Sara      & 3rd                      & Grp     & Real     & 12.1 \\ 
Willow Garage PR2           & ego                      & Grp     & Real     & 11.9 \\ 
RMC RM65           & 3rd                      & Dex     & Real     & 41.3 \\ 

% --- Group 2 ---
\addlinespace[0.8em] 
\multicolumn{5}{l}{\textit{\textbf{Dual-Arm Robots}}} \\ 
\addlinespace[0.2em]
RMC Aida L         & high, wrist$\times$2 & Grp & Real     & 325.7 \\ 

Galaxea R1 Lite    & high, wrist$\times$2 & Grp & Real     & 630.5 \\ 
Agilex Split ALOHA & high, wrist$\times$2 & Grp & Real/Sim & 1099.1 \\ 
Agilex Cobot Magic & high, wrist$\times$2 & Grp & Real     & 399.2 \\ 
Piper              & ego, wrist$\times$2  & Grp & Real/Sim & 904.5 \\ 
 
% --- Group 3 ---
\addlinespace[0.8em]
\multicolumn{5}{l}{\textit{\textbf{Portable Education Arm}}} \\ 
\addlinespace[0.2em]
BeingBeyond D1 & ego           & Dex & Real & 100.0 \\ 
SO101          & ego, wrist$\times$2 & Grp & Real & 194.4 \\ 
 
% --- Group 4 ---
\addlinespace[0.8em]
\multicolumn{5}{l}{\textit{\textbf{Half-Humanoid}}} \\ 
\addlinespace[0.2em]
PND AdamU        & ego                 & Dex     & Real     & 200.0 \\ 
Agibot-G1       & \{ego, wrist\}$\times$2 & Grp/Dex & Real/Sim & 2391.7 \\ 
Leju kuavo 4 LB & ego, wrist$\times$2     & Grp/Dex & Real     & 1198.2 \\ 
AlphaBot 2      & ego, wrist$\times$2     & Grp     & Real     & 13.8 \\ 
Airbot MMK2     & 3rd, wrist$\times$2     & Grp     & Real     & 23.1 \\ 
Galbot G1       & wrist$\times$2          & Grp     & Sim      & 195.8 \\ 
Tianqing A2     & high, wrist$\times$2    & Grp     & Real     & 19.4 \\ 
 
% --- Group 5 ---
\addlinespace[0.8em]
\multicolumn{5}{l}{\textit{\textbf{Humanoid}}} \\ 
\addlinespace[0.2em]
Unitree G1edu-u3 & ego, wrist$\times$2 & Grp/Dex & Real & 135.7 \\ 
Tiankung         & top                 & Grp     & Real & 214.3 \\ 
 
\midrule[\heavyrulewidth] 
 
\multicolumn{4}{l}{\textbf{Total: 30 embodiments}} & \textbf{13817.4} \\ 
\bottomrule
\end{tabular}
\end{table*}


==> table/human_data_list.tex <==
\begin{table*}[h!]
\centering
\caption{The robot data 
used for pretraining Being-H0.5 includes demonstrations from \textbf{29 distinct robotic embodiments} and encompasses over \textbf{11,000 hours}, resulting in \textbf{25.5 million} text token and \textbf{64.1 billion} image training tokens in total.
Episodes are labeled as ``grp'' (parallel gripper) or ``dex'' (dexterous hand), and as ``real'' (collected via real-world teleoperation) or ``sim'' (collected in simulation). The dataset features diverse camera views, varying robotic structures, and a wide range of scenarios.  
This collection represents the most diverse and largest robotic pretraining corpus to date. }
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.1}
\scalebox{0.9}{
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Robot Type} & \textbf{Camera Views} & \textbf{EEF Type} & \textbf{Data Source} & \textbf{Duration (Hours)} \\
    \midrule
    \textbf{Single-Arm Robots} & & & & \\
    \cmidrule(lr){1-1}
    Franka & ego, 3rd$\times$2, wrist & grp \& dex & real \& sim & 2196.4 \\
    Google Robot & ego, 3rd & grp & real \& sim & 597.5 \\
    Kuka-iiwa & ego, 3rd & grp & real \& sim & 169.11 \\
    WidowX & 3rd$\times$2, wrist & grp & real \& sim & 152.6 \\
    Xarm7 Robot & top, 3rd & grp & real \& sim & 297.24 \\
    UR5 & 3rd, wrist & grp & real \& sim & 104.14 \\
    Hello Stretch & ego, 3rd & grp & real & 135.14 \\
    Jaco & 3rd$\times$3 & grp & real \& sim & 97.22 \\
    Kinova3 & 3rd$\times$3 & grp & sim & 98.7 \\
    Sawyer & 3rd & grp & sim & 98.2 \\
    Cobotta & 3rd & grp & real & 5.3 \\
    DLR Sara & 3rd & grp & real & 6.06 \\
    PR2 & ego & grp & real & 5.97 \\
    \midrule
    
    \textbf{Dual-Arm Robots} & & & & \\
    \cmidrule(lr){1-1}
    RMC Aida L & high, wrist$\times$2 & grp & real & 162.87 \\
    Galaxea R1 Lite & high, wrist$\times$2 & grp & real & 630.56 \\
    Agilex Split ALOHA & high, wrist$\times$2 & grp & real \& sim & 1099.05 \\
    Agilex Cobot Magic & high, wrist$\times$2 & grp & real & 194.6 \\
    Piper & ego, wrist$\times$2 & grp & real \& sim & 904.54 \\
    \midrule
    
    \textbf{Portable Arm} & & & & \\
    \cmidrule(lr){1-1}
    BeingBeyond D1 & ego & dex & real & 100 \\
    SO101 & ego, wrist$\times$2 & grp & real & 97.22 \\
    \midrule
    
    \textbf{Half-Humanoid} & & & & \\
    \cmidrule(lr){1-1}
    PND Adam & ego & dex & real & 200 \\
    Agibot-G1 & \{ego, wrist\}$\times$2 & grp \& dex & real \& sim & 2391.67 \\
    Leju kuavo 4 LB & ego, wrist$\times$2 & grp \& dex & real & 1198.15\\
    AlphaBot 2 & ego, wrist$\times$2 & grp & real & 6.94 \\
    Airbot MMK2 & 3rd, wrist$\times$2 & grp & real & 11.55 \\
    Galbot G1 & wrist$\times$2 & grp & sim & 97.96 \\
    Tianqing A2 & high, wrist$\times$2 & grp & real & 9.75 \\
    \midrule
    
    \textbf{Humanoid} & & & & \\
    \cmidrule(lr){1-1}
    Unitree G1edu-u3 & ego, wrist$\times$2 & grp \& dex & real & 67.87 \\
    Tiankung & top & grp & real & 107.13 \\
    \midrule
    
    \textbf{Total: 29 embodiments} & & & & \textbf{11049.63} \\
    \bottomrule
    \end{tabular}
}
\label{tab:robot_data}
\end{table*}


==> table/real_robot_exps.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Real-world success rates (\%) across heterogeneous platforms.} Each task is evaluated over 20 blind trials. Being-H0.5 consistently outperforms baselines across diverse embodiments, with the largest gains on bimanual coordination and few-shot adaptation scenarios.}
\label{tab:real_robot_main}
\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{ll|ccc >{\cellcolor{BlockA!30}}c}
\toprule
\textbf{Platform} & \textbf{Task} & \textbf{Scratch} & \textbf{$\pi_{0.5}$} & \textbf{Being-H0.5} & \textbf{Gain} \\
\midrule
\multirow{6}{*}{\shortstack[l]{\textbf{AdamU} \\ \scriptsize (31 DoF, Bimanual)}} 
    & Bimanual Pick-to-Box & -- & -- & \textbf{--} & -- \\
    & Bimanual Hand-Over   & -- & -- & \textbf{--} & -- \\
    & Pick-to-Drawer       & -- & -- & \textbf{--} & -- \\
    & Flower Arrangement   & -- & -- & \textbf{--} & -- \\
    & Liquid Pouring       & -- & -- & \textbf{--} & -- \\
    & Surface Wiping       & -- & -- & \textbf{--} & -- \\
\cmidrule{2-6}
    & \textit{Subtotal Average} & -- & -- & \textbf{--} & -- \\
\midrule
\multirow{5}{*}{\shortstack[l]{\textbf{Franka-Inspire} \\ \scriptsize (13 DoF, Tabletop)}} 
    & Multi-Bowl Stacking  & -- & -- & \textbf{--} & -- \\
    & Precise Placement    & -- & -- & \textbf{--} & -- \\
    & Block Stacking       & -- & -- & \textbf{--} & -- \\
    & Tool Use (Watering)  & -- & -- & \textbf{--} & -- \\
    & Surface Wiping       & -- & -- & \textbf{--} & -- \\
\cmidrule{2-6}
    & \textit{Subtotal Average} & -- & -- & \textbf{--} & -- \\
\midrule
\textbf{BeingBeyond D1} & Block Stacking & -- & -- & \textbf{--} & -- \\
\midrule
\textbf{Unitree G1} & Flip-and-Scan & -- & -- & \textbf{--} & -- \\
\midrule
\multicolumn{2}{l|}{\textbf{Overall Performance (Mean)}} & -- & -- & \textbf{\cellcolor{BlockA!30}--} & \textbf{+--\%} \\
\bottomrule
\end{tabular}
\end{table}



==> table/sim_libero.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Success rates (\%) on the LIBERO benchmark.} Being-H0.5 is evaluated against a wide range of state-of-the-art VLA models. We report the mean success rate over 50 evaluation episodes per task. Being-H0.5 achieves leading performance on the overall average, with a significant advantage in \texttt{LIBERO-Long}, which requires complex multi-step reasoning. Best results are \textbf{bolded}, and second-best are \underline{underlined}.}
\label{tab:libero_results}
\small
\setlength{\tabcolsep}{8pt}
\resizebox{.8\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
\textbf{Method} & \textbf{L-Spatial} & \textbf{L-Object} & \textbf{L-Goal} & \textbf{L-Long} & \textbf{Average} \\
\midrule
Diffusion Policy \citep{chi2025diffusion} & 78.5 & 87.5 & 73.5 & 64.8 & 76.1 \\
OpenVLA \citep{kim2024openvla} & 84.7 & 88.4 & 79.2 & 53.7 & 76.5 \\
SpatialVLA \citep{qu2025spatialvla} & 88.2 & 89.9 & 78.6 & 55.5 & 78.1 \\
CoT-VLA \citep{zhao2025cotvla} & 87.5 & 91.6 & 87.6 & 69.0 & 83.9 \\
$\pi_0$-Fast \citep{pertsch2025fast} & 96.4 & 96.8 & 88.6 & 60.2 & 85.5 \\
\midrule
GR00T-N1 \citep{nvidia2025gr00t} & 94.4 & 97.6 & 93.0 & 90.6 & 93.9 \\
$\pi_0$ \citep{black2024pi_0} & 98.0 & 96.8 & 94.4 & 88.4 & 94.4 \\
F1 \citep{lv2025f1} & 98.2 & 97.8 & 95.4 & 91.3 & 95.7 \\
InternVLA-M1 \citep{chen2025internvla-m1} & 98.0 & 99.0 & 93.8 & 92.6 & 95.9 \\
Discrete Diffusion VLA \citep{liang2025discrete} & 97.2 & 98.6 & 97.4 & 92.0 & 96.3 \\
$\pi_{0.5}$ \citep{intelligence2025pi05} & 98.8 & 98.2 & 98.0 & 92.4 & 96.9 \\
OpenVLA-OFT \citep{kim2025openvla-oft} & 97.6 & 98.4 & 97.9 & 94.5 & 97.1 \\
X-VLA \citep{zheng2025xvla} & 98.2 & 98.6 & 97.8 & \textbf{97.6} & 98.1 \\
EO1 \citep{qu2025eo1} & \textbf{99.7} & \textbf{99.8} & \underline{99.2} & 94.8 & \underline{98.2} \\
\midrule
\rowcolor{BlockA!20} \textbf{Being-H0.5}(generalist) & 97.0 & 98.2 & 99.0 & 96.2 & 97.6 \\
\rowcolor{BlockA!20} \textbf{Being-H0.5}(specialist) & \underline{99.2} & \underline{99.6} & \textbf{99.4} & \underline{97.4} & \textbf{98.9} \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/sim_robocasa.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Success rates (\%) on the RoboCasa 24-task benchmark}. Being-H0.5 is evaluated across three task categories, averaged over 50 trials per task. Despite using only 224$\times$224 RGB inputs, Being-H0.5 outperforms state-of-the-art 3D-based methods and existing VLAs on the overall average. Best results are \textbf{bolded}, and second-best are \underline{underlined}.}
\label{tab:robocasa_results_refined}
\small
\setlength{\tabcolsep}{6pt}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{llcccc}
\toprule
\textbf{Modality} & \textbf{Method} & \textbf{Pick \& Place} & \textbf{Doors/Drawers} & \textbf{Others} & \textbf{Total Avg.} \\
\midrule
\rowcolor{gray!5} \textit{3D (Multi-modal)} & & & & & \\
3D & 3DA \cite{3d_diffuser_actor} & 0.0 & 2.3 & 13.1 & 5.5 \\
3D & DP3 \cite{Ze2024DP3} & 1.5 & 41.7 & 32.0 & 22.8 \\
3D & GWM \cite{lu2025gwm} & 14.8 & 54.3 & 49.8 & 39.3 \\
\midrule
\rowcolor{gray!5} \textit{RGB-only (Standard)} & & & & & \\
RGB (256$\times$256) & BC \cite{nasiriany2024robocasa} & 4.3 & 47.0 & 42.2 & 28.9 \\
RGB (256$\times$256) & GR00T-N1 \cite{nvidia2025gr00t} & 18.6 & 50.2 & 39.1 & 36.0 \\
RGB (256$\times$256) & $\pi_{0.5}$ \cite{intelligence2025pi05} & 21.5 & 57.8 & 44.9 & 41.4 \\
RGB (256$\times$256) & $\pi_{0}$ \cite{black2024pi_0} & 14.0 & 53.1 & \textbf{58.5} & 42.4 \\
\midrule
\rowcolor{BlockA!20} RGB (224$\times$224) & \textbf{Being-H0.5}(generalist) & \textbf{40} & \textbf{73} & 52 & \underline{53.3} \\
\rowcolor{BlockA!20} RGB (224$\times$224) & \textbf{Being-H0.5}(specialist) & \underline{36} & \underline{71.7} & \underline{57.6} & \textbf{53.9} \\
\bottomrule
\end{tabular}
}
\end{table}

